Husky: A Unified, Open-Source Language Agent for Multi-Step Reasoning

Language agents perform complex tasks by using tools to execute each step precisely. However, most existing agents are based on proprietary models or designed to target specific tasks, such as mathematics or multi-hop question answering. We introduce Husky, a holistic, open-source language agent that learns to reason over a unified action space to address a diverse set of complex tasks involving numerical, tabular, and knowledge-based reasoning. Husky iterates between two stages: 1) generating the next action to take towards solving a given task and 2) executing the action using expert models and updating the current solution state. We identify a thorough ontology of actions for addressing complex tasks and curate high-quality data to train expert models for executing these actions. Our experiments show that Husky outperforms prior language agents across 14 evaluation datasets. Moreover, we introduce HuskyQA, a new evaluation set which stress tests language agents for mixed-tool reasoning, with a focus on retrieving missing knowledge and performing numerical reasoning. Despite using 7B models, Husky matches or even exceeds frontier LMs such as GPT-4 on these tasks, showcasing the efficacy of our holistic approach in addressing complex reasoning problems. Our code and models are available at https://github.com/agent-husky/Husky-v1.

==> unused/abstract.tex <==
Language agents perform complex tasks step-by-step by utilizing tools to execute each step precisely.
However, existing agents are costly to scale, focus on narrow sets of tasks, or require complex inference procedures with task-specific tools.\
We introduce \agent, a unified language agent which solves complex, multi-step reasoning tasks.
%using a multi-task and open-source model that generalizes across tasks and tools. 
 \agent decomposes the problem into a sequence of simpler steps with a single multi-task action generator, and it executes each step with a specialized model or tool for coding, math, web search and general-purpose reasoning.
% For each step, \agent jointly predicts a high-level step along with the recommended tool and executes the step with the tool, iterating over this procedure until it arrives at the final answer.
%Our framework consists of an action generator and several expert models dedicated to coding, math, web search and general-purpose reasoning.
In addition to being open-sourced, \agent is notable for its 1) generalizability across multiple domains spanning numerical, tabular and knowledge-based reasoning, 2) high performance across all evaluation tasks by utilizing state-of-the-art models for its action generator and expert models, and
% efficient two-stage inference where it first jointly generates the high-level step and tool, and then executes the step with the assigned tool, and 
% 3) its ability to apply a minimal set of tools (e.g., code interpreter, web browser) to solve new tasks with competitive performance.
3) its diverse variants consisting of different base models and training sets which help to study the effect of model choice and dataset composition on language agent capabilities.
% We also provide detailed analyses in the effect of model choice and dataset composition on the agent performance.
Furthermore, we present \dataset, a new benchmark which tests a model's ability to identify knowledge it needs to retrieve and perform complex numerical reasoning with the retrieved knowledge.
While even state-of-the-art LMs struggle to answer these questions, \agent retrieves the correct tools and solves the questions successfully.
Our work highlights the challenges in utilizing open-source LMs in an agentic framework and presents several promising directions to improve such systems.
